Blox-Net: Generative Design-for-Robot-Assembly Using VLM Supervision, Physics Simulation, and a Robot with Reset

Generative AI systems have shown impressive capabilities in creating text, code, and images. Inspired by the rich history of research in industrial ''Design for Assembly'', we introduce a novel problem: Generative Design-for-Robot-Assembly (GDfRA). The task is to generate an assembly based on a natural language prompt (e.g., ''giraffe'') and an image of available physical components, such as 3D-printed blocks. The output is an assembly, a spatial arrangement of these components, and instructions for a robot to build this assembly. The output must 1) resemble the requested object and 2) be reliably assembled by a 6 DoF robot arm with a suction gripper. We then present Blox-Net, a GDfRA system that combines generative vision language models with well-established methods in computer vision, simulation, perturbation analysis, motion planning, and physical robot experimentation to solve a class of GDfRA problems with minimal human supervision. Blox-Net achieved a Top-1 accuracy of 63.5% in the ''recognizability'' of its designed assemblies (eg, resembling giraffe as judged by a VLM). These designs, after automated perturbation redesign, were reliably assembled by a robot, achieving near-perfect success across 10 consecutive assembly iterations with human intervention only during reset prior to assembly. Surprisingly, this entire design process from textual word (''giraffe'') to reliable physical assembly is performed with zero human intervention.

==> perturb_table.tex <==
\begin{table*}[h]
\centering
\vspace{0.5em}
\label{table:transposed-evaluation}
{\footnotesize
\begin{tabular}{cccccc}
\toprule
\textbf{Task} & \textbf{Metric} & \textbf{Jigsaw and Shelf} & \textbf{Iron and Shelf} & \textbf{Shoe and Shoerack} \\
\midrule
\multirow{3}{*}{\textbf{Pick and Place}} & \textbf{Max Pick and Place} & 11 & 6 & 8 \\
 & \textbf{Successful Pick Rate} & $21/(24+?)$ & $20/21$ & $25/29$ \\
 & \textbf{Successful Place Rate} & $21/(21+?)$ & $16/21$ & $23/25$ \\
\midrule
\multirow{3}{*}{\textbf{Translation Error}} & \textbf{Mean Translation Error (cm)} & N/A & N/A & N/A \\
 & \textbf{St. Dev. Translation Error (cm)} & N/A & N/A & N/A \\
 & \textbf{Percent Places Within Xcm} & N/A & N/A & N/A \\
\bottomrule
\end{tabular}
}
\caption{Evaluation results of pairwise comparisons between (AD) and other baselines with GPT-4-Turbo as judge.}
\vspace{-0.5em}
\end{table*}

